What do End-to-End Speech Models Learn about Speaker, Language and Channel Information? A Layer-wise and Neuron-level Analysis

Deep neural networks are inherently opaque and challenging to interpret. Unlike hand-crafted feature-based models, we struggle to comprehend the concepts learned and how they interact within these models. This understanding is crucial not only for debugging purposes but also for ensuring fairness in ethical decision-making. In our study, we conduct a post-hoc functional interpretability analysis of pretrained speech models using the probing framework [1]. Specifically, we analyze utterance-level representations of speech models trained for various tasks such as speaker recognition and dialect identification. We conduct layer and neuron-wise analyses, probing for speaker, language, and channel properties. Our study aims to answer the following questions: i) what information is captured within the representations? ii) how is it represented and distributed? and iii) can we identify a minimal subset of the network that possesses this information? Our results reveal several novel findings, including: i) channel and gender information are distributed across the network, ii) the information is redundantly available in neurons with respect to a task, iii) complex properties such as dialectal information are encoded only in the task-oriented pretrained network, iv) and is localised in the upper layers, v) we can extract a minimal subset of neurons encoding the pre-defined property, vi) salient neurons are sometimes shared between properties, vii) our analysis highlights the presence of biases (for example gender) in the network. Our cross-architectural comparison indicates that: i) the pretrained models capture speaker-invariant information, and ii) CNN models are competitive with Transformer models in encoding various understudied properties.

==> sections/bck_intro.tex <==
\section{Introduction}
\label{sec:intro}


Deep Neural Networks have constantly pushed the state-of-the-art in speech technologies, for example automatic speech recognition (ASR) \cite{amodei2016deep,miao2015eesen,pratap2019wav2letter++,chan2016listen,chowdhury2021onemodel,ali2021csmodel}, pretrained speech transformers \cite{baevski2020wav2vec,liu2020mockingjay,liu2020tera,chi2020audio}, dialect, language and speaker identification \cite{jin2017end, trong2016deep, heigold2016end, nagrani2017voxceleb, snyder2017deep, shon2018convolutional, snyder2018x} models,
along with other fields in Artificial Intelligence,  including Natural Language Processing (NLP) \cite{deng2018deep} and Computer Vision (CV) \cite{voulodimos2018deep}. While end-to-end deep architectures are simple, elegant, and provide a flexible training mechanism, they are inherently black-boxes. Unlike the traditional models, they lack the explanation of what information is captured within the learned representations, and how it is encoded and used in the decision process. This opaqueness hinders practitioners from understanding the internal mechanics of the models and the %causation process 
causal effect, which is critical for debugging, ethical decision making, and fairness in these systems \cite{doshi2017towards,lipton2018mythos}. 
To this end, researchers have investigated deep neural models for auxiliary knowledge they encode in the learned representation through probing classifiers \cite{dalvi2019one, dalvi2019neurox,belinkov2017neural,dalvi2017understanding}, via visualizations \cite{zhang2018visual,zeiler2014visualizing}, through ablation studies \cite{sheikholeslami2021autoablation}, and using unsupervised methods \cite{harwath2017learning}.

% Work done using \emph{Diagonostic Classifiers} analyze representations at the level of individual layers \cite{elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does}, attention heads \cite{ghader2017does} and a more fine-grained neuron level \cite{dalvi2019one,durrani2020analyzing, qian2016analyzing}. These studies reveal interesting findings such as how different linguistic properties (such as morphology and syntax) are captured in different parts of the network, and how certain properties are more localized or distributed than others. 
% % \sout{\textit{(a)} its learning capability; \textit{(b)} the granularity of individual layers; and finally \textit{(c)} the role of individual neurons; using visualization \cite{zhang2018visual,zeiler2014visualizing}, model diagnosis \cite{ribeiro2016should}, explanatory graphs \cite{zhang2018interpreting}, proxy classifier \cite{dalvi2019one, dalvi2019neurox,belinkov2017neural,dalvi2017understanding} along with explainable models \cite{sabour2017dynamic}.}


% While some work has been done to interpret representations in the speech models \cite{beguvs2021interpreting, elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does,becker2018interpreting}, no prior work has been carried to do a neuron-level analysis. Analyzing individual neurons facilitates a deeper understanding of the network \cite{girshick2016, nguyen2016synthesizing, bau2017network,dalvi2019one,durrani2020analyzing, qian2016analyzing,shi2016neural} and entails many potential benefits such as manipulating system's output \cite{indivdualneuron:arxiv19} while debasing the network w.r.t certain property (like gender or racial elements), model distillation and compression \cite{rethmeier2019txray,frankle2018lottery}, domain adaptation \cite{gu2021pruningthenexpanding},  feature selection for downstream tasks \cite{dalvi2020analyzing} and guiding architectural search etc. %To %enrich speech community with 
% %develop a better understanding of the learned representations, %model's prediction, the encoded information 
% %along with presence of bias and redundancy, we carry a layer and neuron-level analysis on the speech models.

% Speech signals are long, have variable lengths and are of complex hierarchical structure. 
% Learning meaningful information in such continuous modality is difficult.
%  specially when the models need to integrate information from larger time spans
Speech signals are long, have variable lengths, and exhibit complex hierarchical structures on different time scales.\footnote{For instance, syllables are made up of phonemes that temporally extend over a few milliseconds} These properties of speech make
learning meaningful information challenging. Moreover, the environmental\footnote{e.g. \textit{channel information} -- signal recording and transmission quality of the speech.} and speaker\footnote{\textit{voice identity, gender, age, language.}} influenced variables in speech models impose different characteristics on the acoustic input, resulting in added complexity, thus making it harder to understand models' decisions. For instance, the speaker recognition (SR) systems process extremely personal data,\footnote{carrying individual identity} which is highly susceptible to biases \cite{6613025}, therefore it is fundamental that we understand what other factors like gender, race, accent, microphones are hindering the model's decision. 

% is a neccesity to understand the 

% process extremely personal data, carrying individual identity. This makes the SR model highly susceptible to bias and it is a necessity  


% susceptible to perpetrate discrimination
% does the model learn speaker identity or the environmental properties such as a microphone? 

A prominent framework for probing whether a neural network model has captured certain phenomenon is the \emph{Diagonostic Classifiers} \cite{belinkov2017neural} which has been extensively used to analyze representations at the level of individual layers \cite{elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does}, attention heads \cite{ghader2017does} and a more fine-grained neuron level \cite{dalvi2019one,durrani2020analyzing, qian2016analyzing}. These studies reveal interesting findings such as how different linguistic properties (such as morphology and syntax) are captured in different parts of the network, and how certain properties are more localized or distributed than others. While some work has been done to interpret representations in the speech models \cite{beguvs2021interpreting, elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does,becker2018interpreting}, no prior work has been carried to do a neuron-level analysis. Analyzing individual neurons facilitates a deeper understanding of the network \cite{girshick2016, nguyen2016synthesizing, bau2017network,dalvi2019one,durrani2020analyzing, qian2016analyzing,shi2016neural} and entails many potential benefits such as manipulating system's output \cite{indivdualneuron:arxiv19} while debasing the network w.r.t certain property (like gender or racial elements), model distillation and compression \cite{rethmeier2019txray,frankle2018lottery}, domain adaptation \cite{gu2021pruningthenexpanding},  feature selection for downstream tasks \cite{dalvi2020analyzing} and guiding architectural search etc.

% #Questions we aim to answer
In this study, we focus on post-hoc functional interpretability of pretrained speech models. 
We carry a layer-wise and fine-grained neuron-level analysis on the pretrained speech models for i) speaker: gender and voice identity, ii) language and its dialectal variants, and iii) channel information, using utterance-level representation. We carry our study with the following research questions:
\textbf{RQ1:} %Is the understudied information (e.g. channel) captured in the network's learned representation? 
Does the end-to-end speech models capture different properties (e.g. gender, channel or speaker information)?
\textbf{RQ2:} Where in the network is it preserved and how localized or distributed is it?
\textbf{RQ3:} Can we extract a minimal number of neurons that can represent the same information?  and \textbf{RQ4:} How do the learning patterns changes across different pretrained models?

% #how we want to achieve it

We use a framework based on probing classifiers \cite{hupkes2018visualisation,conneau2018you}. The idea is to extract the representations (of speech utterances) from the understudied pretrained model and train an auxiliary classifier towards predicting the studied properties. The accuracy of the classifier serves as a proxy to the quality of the learned representation with respect to that property. We train classifiers using different layers to carry our layer-wise analysis and do a %more 
fine-grained analysis by probing for neurons that capture these properties.


% #what we used
We investigate 4 pretrained end-to-end architectures: 2 CNN  architectures trained towards the task of speaker recognition and dialect identification, 
and 2 Transformer architectures trained to reconstruct the masked signal. The choice of architectures was driven by the fact that these models have shown state-of-the-art performances in different speech tasks. Also comparing CNNs to the recently emerged transformer architecture provides interesting cross-architectural analysis. Our cross architectural analysis shows that:

 \begin{itemize}
 \setlength\itemsep{0em}
    
    
    \item \textit{Task complexity and Minimal neuron set:} Less neurons ($\approx$ 1-5\%) are required to encode simple properties (e.g. gender) unlike the complex properties such as regional dialect identification or voice identification. ($\rightarrow$ RQ1, RQ3)
    
    \item \textit{Task-specific Redundancy:} Layer-wise and neuron-level task-specific redundancy is observed in capturing gender and channel information. These %information 
    phenomena are distributed throughout the network encoding redundant information, thus can be captured with small number of neurons from any part of the network. Such redundancy is also noticed %in the case of %encapsulating 
    when encoding language property ($\rightarrow$ RQ3)
    
    \item \textit{Localized vs Distributive:} The salient neurons are localised in the final layers of the pretrained models, indicating that the deeper neurons of the network are more informative than %its predecessor 
    and capture more abstract information. This observation %is seen 
    was true for both simple and complex tasks ($\rightarrow$ RQ2)
    
    \item \textit{Robustness:} Most of the pretrained models learn speaker-invariant information ($\rightarrow$ RQ1, RQ4) 
    
    
    \item \textit{Polysemous Neurons:} %The salient neurons are sometimes shared between multiple properties in a pretrained model. 
    Neurons are multivariate in nature and shared among properties. For example, some neurons were found to be salient for both voice identity, and gender properties ($\rightarrow$ RQ2, RQ3) 
    
    \item \textit{Bias:} %It is possible 
    We were able to %pinpoint
    highlight neurons responsible for sensitive information (e.g., gender). This can be potentially %used 
    useful in future to mitigate model bias ($\rightarrow$ RQ3) 
    
    \item \textit{Pretrained Models for Transfer learning:} Pretrained CNNs give comparable, sometimes even outperforms, the speech transformers and can %easily 
    be used as a viable feature extractor (or for fine-tuning) in the downstream tasks. In line with \cite{tay2021pretrained}, our findings suggest the potential of re-using large CNNs as pretrained network with similar efficacy as the pretrained speech transformers. ($\rightarrow$ RQ4) 
    
    \end{itemize}
 
\noindent To the best of our knowledge, \textbf{this work is the first attempt that carries a layer-wise and fine-grained neuron-level analysis on the pretrained CNNs and Transformers speech models.} 






% \nd{What is the role of the below paragraphs? If they are findings they should be part of the bullets. Put a bullet on what was the finding from redundancy analysis and then a bullet about finding about CNN vs speech transformer and remove the paragraph below}
 
%  \noindent Moreover, our study indicates, using the size of the minimal neuron set along with top/random neurons, we can infer the presence/absence of property-based network redundancy ($\rightarrow$ RQ3). Furthermore, our findings suggest that pretrained CNNs give comparable (even outperforms) the speech transformers and can easily be used as a feature extractor (or for fine-tuning) in the downstream tasks. In line with \cite{tay2021pretrained}, our findings suggest the potential of re-using large CNNs as pretrained network with similar efficacy as the pretrained speech transformers. 

 
%  Our study also reveals an interesting relation between the size of the minimal neuron set, and task complexity and network redundancy.

% #potential application

% : \textit{whether} speaker, channel, language and its variants -- information are encoded in the network, if so \textit{where} they are located and \textit{how distributed} the information is? And most importantly, \textit{can we extract a small subset of neurons} to represent the same information?

% \nd{The above is redundant - I would remove it}

% #our contribution is answering
% Our work also provides a preliminary study for identifying layers and neurons responsible for sensitive information -- such as channel \hll{and} gender. \hll{Such an analysis can be useful} \sout{and use it} to mitigate \sout{such} model bias, \sout{to lessen their} \hll{for reducing its} effect on model performance and enhance model generalisation capabilities. \sout{Such an analysis has many} \hll{Other} potential applications \hll{include} \sout{such as} efficient feature selection for the downstream task,
% model distillation and compression \cite{rethmeier2019txray} - by removing non-contributing neurons and manipulation by controlling neurons in the network \cite{indivdualneuron:arxiv19}.

% To the best of our knowledge, this is the first attempt to a layer-wise and a fine-grained neuron-level analysis on the pretrained speech models. 

% \nd{This last paragraph should be reordered. You should talk about what are benefits of neuron analysis and then narrow it down to the scope of this work rather than saying this is what we did but neuron analysis can be done for all this other stuff. I think it should fit in paragraphs 25-30 (in pdf)}

==> sections/introductionOld.tex <==
\section{Introduction}
\label{sec:intro}

Deep Neural Networks have constantly pushed the state-of-the-art in speech technologies, for example automatic speech recognition (ASR) \cite{amodei2016deep,miao2015eesen,pratap2019wav2letter++,chan2016listen,chowdhury2021onemodel,ali2021csmodel}, pretrained speech transformers \cite{baevski2020wav2vec,liu2020mockingjay,liu2020tera,chi2020audio}, dialect, language and speaker identification \cite{jin2017end, trong2016deep, heigold2016end, nagrani2017voxceleb, snyder2017deep, shon2018convolutional, snyder2018x} models,
along with other arenas of Artificial Intelligence, including Natural Language Processing (NLP) \cite{deng2018deep} and Computer Vision (CV) \cite{voulodimos2018deep}. While end-to-end deep architectures are simple and elegant, and provide a flexible training mechanism, they are inherently black-boxes. Unlike the traditional models, they lack the explanation of what information is captured within the learned representations, and how it is %encoded and 
used in the decision process. This opaqueness hinders practitioners from understanding the internal mechanics of the models and the %causation process 
causal effect, which is critical for debugging, ethical decision making, and fairness in these systems \cite{doshi2017towards,lipton2018mythos}. 
To this end, researchers have investigated deep neural models for auxiliary knowledge they encode in the learned representation through probing classifiers \cite{dalvi2019one, dalvi2019neurox,belinkov2017neural,dalvi2017understanding}, via visualizations \cite{zhang2018visual,zeiler2014visualizing}, through ablation studies \cite{sheikholeslami2021autoablation}, and using unsupervised methods \cite{harwath2017learning}.

% Work done using \emph{Diagonostic Classifiers} analyze representations at the level of individual layers \cite{elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does}, attention heads \cite{ghader2017does} and a more fine-grained neuron level \cite{dalvi2019one,durrani2020analyzing, qian2016analyzing}. These studies reveal interesting findings such as how different linguistic properties (such as morphology and syntax) are captured in different parts of the network, and how certain properties are more localized or distributed than others. 
% % \sout{\textit{(a)} its learning capability; \textit{(b)} the granularity of individual layers; and finally \textit{(c)} the role of individual neurons; using visualization \cite{zhang2018visual,zeiler2014visualizing}, model diagnosis \cite{ribeiro2016should}, explanatory graphs \cite{zhang2018interpreting}, proxy classifier \cite{dalvi2019one, dalvi2019neurox,belinkov2017neural,dalvi2017understanding} along with explainable models \cite{sabour2017dynamic}.}


% While some work has been done to interpret representations in the speech models \cite{beguvs2021interpreting, elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does,becker2018interpreting}, no prior work has been carried to do a neuron-level analysis. Analyzing individual neurons facilitates a deeper understanding of the network \cite{girshick2016, nguyen2016synthesizing, bau2017network,dalvi2019one,durrani2020analyzing, qian2016analyzing,shi2016neural} and entails many potential benefits such as manipulating system's output \cite{indivdualneuron:arxiv19} while debasing the network w.r.t certain property (like gender or racial elements), model distillation and compression \cite{rethmeier2019txray,frankle2018lottery}, domain adaptation \cite{gu2021pruningthenexpanding},  feature selection for downstream tasks \cite{dalvi2020analyzing} and guiding architectural search etc. %To %enrich speech community with 
% %develop a better understanding of the learned representations, %model's prediction, the encoded information 
% %along with presence of bias and redundancy, we carry a layer and neuron-level analysis on the speech models.

% Speech signals are long, have variable lengths and are of complex hierarchical structure. 
% Learning meaningful information in such continuous modality is difficult.
%  specially when the models need to integrate information from larger time spans


% is a neccesity to understand the 

% process extremely personal data, carrying individual identity. This makes the SR model highly susceptible to bias and it is a necessity  


% susceptible to perpetrate discrimination
% does the model learn speaker identity or the environmental properties such as a microphone? 

A prominent framework for probing is the \emph{Diagonostic Classifiers} \cite{belinkov2017neural} which has been extensively used to analyze representations at the level of individual layers \cite{elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does}, attention heads \cite{ghader2017does} and a more fine-grained neuron level \cite{dalvi2019one,durrani2020analyzing, qian2016analyzing}. These studies reveal interesting findings such as how different linguistic properties (such as morphology and syntax) are captured in different parts of the network, and how certain properties are more localized or distributed than others. 
% --- While some work has been done to interpret representations in the speech models \cite{beguvs2021interpreting, elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does,becker2018interpreting}, no prior work has been carried to do a neuron-level analysis. 
Moreover, probing paradigm has been used to analyze individual neurons, facilitating a deeper understanding of the network \cite{girshick2016, nguyen2016synthesizing, bau2017network,dalvi2019one,durrani2020analyzing, qian2016analyzing,shi2016neural}, and entails many potential benefits such as manipulating system's output \cite{indivdualneuron:arxiv19} while debasing the network w.r.t certain property (like gender or racial elements), model distillation and compression \cite{rethmeier2019txray,frankle2018lottery}, domain adaptation \cite{gu2021pruningthenexpanding},  feature selection for downstream tasks \cite{dalvi2020analyzing} and guiding architectural search etc.




In this study, we focus our efforts on studying pretrained speech models. Understanding speech models are challenging since the input signals are long, with variable lengths, and exhibit complex hierarchical structures on different time scales.\footnote{For instance, syllables are made up of phonemes that temporally extend over a few milliseconds} Moreover, the environmental\footnote{e.g. \textit{channel information} -- signal recording and transmission quality of the speech.} and speaker\footnote{\textit{voice identity, gender, age, language.}} influenced variables in speech models impose different characteristics on the acoustic input, resulting in added complexity, making it harder to understand models' decisions. 
For example, in speaker recognition (SR) systems, the model process extremely personal data,\footnote{carrying individual identity} and is highly susceptible to biases \cite{6613025}, therefore it is fundamental that we study and interpret what other factors like gender, race, accent, microphones are hindering the model's decision. While some work has been done to interpret representations in the speech models \cite{beguvs2021interpreting, elloumi2018analyzing, chowdhury2020does,shah2021all,wang2017does,becker2018interpreting}, no prior work has been carried to do a fine-grained neuron-level analysis.

% An example of such a speech model is the speaker recognition (SR) systems, which process extremely personal data,\footnote{carrying individual identity} and is highly susceptible to biases \cite{6613025}, therefore it is fundamental that we understand what other factors like gender, race, accent, microphones are hindering the model's decision. 



% #Questions we aim to answer
Therefore, we focus on post-hoc functional interpretability of pretrained speech models. 
We carry a layer-wise and fine-grained neuron-level analysis on the pretrained speech models for i) speaker: gender and voice identity, ii) language and its dialectal variants, and iii) channel information, using utterance-level representation. We carry our study with the following research questions:
\textbf{RQ1:} %Is the understudied information (e.g. channel) captured in the network's learned representation? 
Does the end-to-end speech models capture different properties (e.g. gender, channel or speaker information)?
\textbf{RQ2:} Where in the network is it represented and how localized or distributed is it?

% #how we want to achieve it

We use aforementioned framework based on probing classifiers \cite{hupkes2018visualisation,conneau2018you}. The idea is to extract the representations (of speech utterances) from the understudied pretrained model and train an auxiliary classifier towards predicting the studied properties. The accuracy of the classifier serves as a proxy to the quality of the learned representation with respect to that property. We train classifiers using different layers to carry our layer-wise analysis and do a %more 
fine-grained analysis by probing for neurons that capture these properties.


% #what we used
We investigate 4 pretrained end-to-end architectures: 2 CNN  architectures trained towards the task of speaker recognition and dialect identification, 
and 2 Transformer architectures trained to reconstruct the masked signal. The choice of architectures was driven by the fact that these models have shown state-of-the-art performances in different speech tasks. Also comparing CNNs to the recently emerged transformer architecture provides interesting cross-architectural analysis. Our cross architectural analysis shows that:

 \begin{itemize}
 \setlength\itemsep{0em}
    
    
    \item \textit{Task complexity and Minimal neuron set:} Less neurons ($\approx$ 1-5\%) are required to encode simple properties (e.g. gender) unlike the complex properties such as regional dialect identification or voice identification. %($\rightarrow$ RQ1, RQ3)
    
    \item \textit{Task-specific Redundancy:} Layer-wise and neuron-level task-specific redundancy is observed in capturing gender and channel information. These %information 
    phenomena are distributed throughout the network encoding redundant information, thus can be captured with small number of neurons from any part of the network. Such redundancy is also noticed %in the case of %encapsulating 
    when encoding language property %($\rightarrow$ RQ3)
    
    \item \textit{Localized vs Distributive:} The salient neurons are localized in the final layers of the pretrained models, indicating that the deeper neurons of the network are more informative than %its predecessor 
    and capture more abstract information. This observation %is seen 
    was true for both simple and complex tasks %($\rightarrow$ RQ2)
    
    \item \textit{Robustness:} Most of the pretrained models learn speaker-invariant information %($\rightarrow$ RQ1, RQ4) 
    
    
    \item \textit{Polysemous Neurons:} %The salient neurons are sometimes shared between multiple properties in a pretrained model. 
    Neurons are multivariate in nature and shared among properties. For example, some neurons were found to be salient for both voice identity, and gender properties %($\rightarrow$ RQ2, RQ3) 
    
    \item \textit{Bias:} %It is possible 
    We were able to %pinpoint
    highlight neurons responsible for sensitive information (e.g., gender). This can be potentially %used 
    useful in future to mitigate model representation bias %($\rightarrow$ RQ3) 
    
    \item \textit{Pretrained Models for Transfer learning:} Pretrained CNNs give comparable, sometimes even outperforms, the speech transformers and can %easily 
    be used as a viable feature extractor (or for fine-tuning) in the downstream tasks. In line with \cite{tay2021pretrained}, our findings suggest the potential of re-using large CNNs as pretrained network with similar efficacy as the pretrained speech transformers. %($\rightarrow$ RQ4) 
    
    \end{itemize}
 
\noindent To the best of our knowledge, \textbf{this work is the first attempt that carries a layer-wise and fine-grained neuron-level analysis on the pretrained CNNs and Transformers speech models.} 






% \nd{What is the role of the below paragraphs? If they are findings they should be part of the bullets. Put a bullet on what was the finding from redundancy analysis and then a bullet about finding about CNN vs speech transformer and remove the paragraph below}
 
%  \noindent Moreover, our study indicates, using the size of the minimal neuron set along with top/random neurons, we can infer the presence/absence of property-based network redundancy ($\rightarrow$ RQ3). Furthermore, our findings suggest that pretrained CNNs give comparable (even outperforms) the speech transformers and can easily be used as a feature extractor (or for fine-tuning) in the downstream tasks. In line with \cite{tay2021pretrained}, our findings suggest the potential of re-using large CNNs as pretrained network with similar efficacy as the pretrained speech transformers. 

 
%  Our study also reveals an interesting relation between the size of the minimal neuron set, and task complexity and network redundancy.

% #potential application

% : \textit{whether} speaker, channel, language and its variants -- information are encoded in the network, if so \textit{where} they are located and \textit{how distributed} the information is? And most importantly, \textit{can we extract a small subset of neurons} to represent the same information?

% \nd{The above is redundant - I would remove it}

% #our contribution is answering
% Our work also provides a preliminary study for identifying layers and neurons responsible for sensitive information -- such as channel \hll{and} gender. \hll{Such an analysis can be useful} \sout{and use it} to mitigate \sout{such} model bias, \sout{to lessen their} \hll{for reducing its} effect on model performance and enhance model generalisation capabilities. \sout{Such an analysis has many} \hll{Other} potential applications \hll{include} \sout{such as} efficient feature selection for the downstream task,
% model distillation and compression \cite{rethmeier2019txray} - by removing non-contributing neurons and manipulation by controlling neurons in the network \cite{indivdualneuron:arxiv19}.

% To the best of our knowledge, this is the first attempt to a layer-wise and a fine-grained neuron-level analysis on the pretrained speech models. 

% \nd{This last paragraph should be reordered. You should talk about what are benefits of neuron analysis and then narrow it down to the scope of this work rather than saying this is what we did but neuron analysis can be done for all this other stuff. I think it should fit in paragraphs 25-30 (in pdf)}

==> sections/toc.tex <==
% \section{Introduction}
% \label{sec:intro}

% \section{Related Work}
% \label{sec:related}

% \section{Methodology}
% \label{sec:methods}
% % \subsection{Sentence Level Representation}
% \subsection{Proxy Classifier}
% \subsection{Fine-grained Neuron Analysis}
% \subsubsection{Neuron Ranking}
% \subsubsection{Efficacy of the Ranking}
% \subsubsection{Minimal Neuron Set}
% \subsubsection{Neuron Distribution}
% \subsection{Evaluation Measures}
% \subsubsection{Layer-wise Ablation}
% \subsubsection{Neuron Ablation}
% \subsubsection{Control Tasks}

% \section{Experimental Setup}
% \label{sec:expsetup}
% \subsection{Pre-trained Models}
% \label{ssec:models}
% \subsection{Proxy Tasks}
% \label{ssec:probing}
% \subsubsection{T1 - Gender Classification (GC)}
% \subsubsection{T2 - Speaker Verification (SV)}
% \subsubsection{T3 - Language Identification (LID)} 
% \subsubsection{T4 - Regional Dialect Classification (DID)}
% \subsubsection{T5 - Channel Classification (CC)}
% \subsection{Classification}
% \label{ssec:models}


\section{Results and Discussion}
\label{sec:result}
\subsection{Speaker Information} 
\subsubsection{T1: Gender Classification, GC}
\subsubsection{T2: Speaker Verification, SV}
\subsection{Language Information} 
\subsubsection{T3: Language Identification, LID}
\subsubsection{T4: Regional Dialect Identification, DID}
\subsection{Channel Information} 
\subsection{Key Observations}
\subsection{Limitations}

\section{Conclusion}
\label{sec:concl}

Our finding suggests that channel and gender information are omnipresence and requires a small subset of neuron unlike the voice identity information, which in presented in last layer of SRE model . The neurons (50-75\%) representing the voice identity are also shared with other properties mainly gender, and language. For language and dialectal information a small number of salient neurons are sufficient, in CNN-architecture, indicating the redundancy in the networks. We also observed how the size/parameters of the speech transformer contribute in encoding the information. We also discuss the relation between the size of the minimal neuron set with the task complexity and the presence of information. We re-confirm the findings inferring the lower layers of the network act as feature extractor and upper layers as task-oriented classifier. 


signaling the task simplicity. 
As for the voice identity, the information is captured in the last layer of speaker recognition model utilising majority of the neurons. Furthermore, our studies showed the neurons encoding voice identity are also shared with other properties mainly gender, and language.
From probing the language and dialectal information, we observed CNN architectures capture the information using a small number of salient neurons, which indicate the presence of the redundancy in the network. We have also observed how hard it is for a small pre-trained transformer architecture, without any supervision, to encode language and dialect information and how increasing the model parameters can help.
Our study also showcase how the size of the minimal neuron set represent the task complexity and the presence of information. In addition, we re-confirm the findings inferring the lower layers of the network act as feature extractor and does not always encode task-oriented properties. Nonetheless, they are important for capturing general and meaningful representations that can encapsulate the structure of the high dimensional input signal. 


